Grammar Based Directed Testing of Machine Learning Systems

The massive progress of machine learning has seen its application over a variety of domains in the past decade. But how do we develop a systematic, scalable and modular strategy to validate machine-learning systems? We present, to the best of our knowledge, the first approach, which provides a systematic test framework for machine-learning systems that accepts grammar-based inputs. Our OGMA approach automatically discovers erroneous behaviours in classifiers and leverages these erroneous behaviours to improve the respective models. OGMA leverages inherent robustness properties present in any well trained machine-learning model to direct test generation and thus, implementing a scalable test generation methodology. To evaluate our OGMA approach, we have tested it on three real world natural language processing (NLP) classifiers. We have found thousands of erroneous behaviours in these systems. We also compare OGMA with a random test generation approach and observe that OGMA is more effective than such random test generation by up to 489%.

==> response.tex <==
\section*{Associate Editor Comments for Grammar Based Directed Testing of Machine Learning Systems}
\label{sec:intro}

We thank the associate editor for the comment. We have addressed this 
comment in the revised version. For the sake of clarity, we have also 
included the reviewer comments from the previous revision, as the 
comments from the associate editor was related to those comments. 

\section*{Associate Editor Comments}
\label{sec:overview-r}
\textit{\textbf {Comment \#1:}
I thank the authors for their extensive rebuttal in the appendix. 
However, what I'd like to see is a version of the revised manuscript 
clearly highlighting these minor revisions. As it stands it's difficult 
for me how the reviewer comments are addressed in the paper. Also, 
please try to incorporate some the rebuttal text into the manuscript 
itself. So instead of just responding to the reviewers in a document 
that no one (except me) will see, put them in the manuscript so that 
future readers get a better picture of the arguments made against 
some of the shortcomings. Again, please clearly indicate in the 
manuscript the changes. Therefore, I'm returning the paper as a 
Minor Revision again.}

\smallbreak
%\todo{
\textit{\textbf{Response \#1:}} Thanks for the comment. We have now 
integrated the relevant text from all our responses in the revised 
main paper. For the sake of clarity, we have also included the 
reviewer comments that appeared in the previous version. In the 
response to the reviewer comments, we have used {\em blue} color 
text to indicate that the respective text also appears in the revised 
version of our paper. In the response, we have also mentioned the 
exact place in the main paper where the response text appears. The 
respective changes in the revised version of the paper are also 
highlighted in blue for cross checking. We hope that the revised 
version incorporates all our responses satisfactorily in the main paper 
for future readers. 


\section*{Review Comments from the previous revision}

%\revise{
In this section, we will go through the reviewer comments and outline 
how these comments and concerns were addressed in the revised paper.
%}



\subsection*{Response for Reviewer \#1}
%\revise{
\textit{\textbf {Comment \#1:} For the motivation to design OGMA, the 
authors emphasize the importance to explore as many as erroneous instances 
in a confined subspace, which would be more helpful to fix the bug. 
However, as shown in the $\mu$RQ, it is when augmenting the training 
dataset by 15\% with the erroneous inputs that it achieves the largest 
reduction in errors, not when augmenting by 25\%. The experiment results 
raised my concern on the motivation to have a directed testing tool like 
OGMA.
 }
%}

\smallbreak
%\todo{
\textit{\textbf{Response \#1:}}
%}
Thanks for the comment. In our work, we do not mean that all 
the erroneous inputs should be added to the training set for improving 
the model. As also observed in our experiments that naively adding the 
erroneous inputs to the training set may increase the error rate. To 
clarify why it is necessary to generate many erroneous inputs, we have 
added the following text in the revised paper (see \autoref{sec:results}, 
``Results" under $\mu$RQ, column 2, second paragraph): 
%
\newrevise{Although in certain cases it might be possible to repair the 
machine-learning (ML) model with few representative inputs, we believe 
it is necessary to generate a significant number of erroneous inputs 
(when possible). This is because of \textbf{two} reasons. 
Firstly, the erroneous 
inputs generated by \FT can be used to retrain the underlying ML algorithm 
and reduce its erroneous behaviour. The exact percentage of inputs that 
need to be added may depend on the application and the ML algorithm. 
In our evaluation, for example, augmenting the training set by 15\% with 
the error inducing inputs led to the largest reduction in errors. Secondly, 
even though the repair might be achieved by a few representative error 
inputs, it is crucial to test the repaired model with a substantial number 
of error inducing inputs generated by \FT. This is to check whether the 
repaired model indeed reduced the error rate. In the absence of a 
substantial number of error inducing inputs, the designer will not be able 
to validate a repaired model.}

%\newrevise{
It is important to note that the generated errors are not present 
in the training dataset. Additionally, if the user wishes to stop the 
test generation after a given number of iterations are run, it is possible 
to do that in the current design of \FT.%}

\textit{\textbf {Comment \#2:} In general, the robustness property is 
considered regarding a type of “similarity” definition, with which two 
similar samples could have similar predictions. For NLP tasks, it is 
usually the semantic similarity, and synonym replacement is often used to 
retain such similarity.}


\textit{
With the explanations from the authors, I understand that OGMA does not 
need to keep the semantic similarity because it does not rely on such 
similarity to guarantee the newly generated samples to have the same ground 
truth with the original seed, and to further determine whether they are 
erroneous. Actually, the authors relax the restriction of the space to 
search for errors, which should be a superset of the robustness defined 
area.}

\textit{
However, this raises some concern on the scope of the errors located by 
such a directed testing scheme. Are these errors caused by the same defect 
of the models? If not, I think the motivation to find more errors with OGMA 
becomes much weaker. }

\textit{
Moreover, such mutations will make the newly generated samples wild, i.e., 
without truth label, which will hinder the practical usage of OGMA. I will 
comment more on this point in the usability part.
 }
%}

\smallbreak
%\todo{
\textit{\textbf{Response \#2:}}
Thanks for the comment. To clarify this aspect, we have added the following 
text in the revised paper (\autoref{sec:conclusion}, ``Conclusion", second paragraph): 

\newrevise{\FT directs the search process in the input space to maximize the 
number of errors found. These errors may not necessarily be due to the same 
defect of the model. Thus, we believe that \FT is a powerful tool to discover 
erroneous inputs that may be caused due to a variety of defects embodied 
within the model. In other words, \FT should be used as a testing tool for 
NLP models to discover errors. However, in its current state, \FT is not capable 
to pin down the root cause in the model for a given erroneous input. This requires 
further development in the fault localization research.} 

We had also clarified the following in the conclusion:  In future, we plan to 
extend the capability of OGMA to automatically localise the cause of errors 
discovered in these machine learning based natural language processing models.

\textit{\textbf {Comment \#3.1:}
The missing label problem of the newly generated errors could be a major 
concern for the users of OGMA. In the $\mu$RQ, the authors assume there 
exits an oracle to label the errors, which is not possible in real world ML 
applications. Also, without the truth labels, the errors are hard to be 
confirmed to be real errors (to one of the two models under test), and can 
also not be used to do the retraining.
}


\begin{table*}
\caption{Number of errors for Sentiment analysis using Rosette and Google}
\label{table:rq6-errors-response}
\centering
\arrayrulecolor{black}
\setlength{\fboxrule}{3pt}
\fcolorbox{blue}{white}{
\begin{tabular}{!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-10}
\multicolumn{1}{!{\color{black}\vrule}l!{\color{black}\vrule}}{} & \multicolumn{3}{c!{\color{black}\vrule}}{\FT} & \multicolumn{3}{c!{\color{black}\vrule}}{Random} & \multicolumn{3}{c!{\color{black}\vrule}}{\FT - No Backtrack}  \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-10}
Grammar                                                          & \#inputs & \#errs & $err_r$                          & \#inputs & \#errs & $err_r$                        & \#inputs & \#errs & $err_r$                                          \\ 
\hline
A                                                                & 195      & 160    & 0.82                           & 195      & 59     & 0.30                         & 196      & 83     & 0.42                                           \\ 
\hline
B                                                                & 194      & 173    & 0.89                           & 197      & 71     & 0.36                         & 197      & 100    & 0.51                                           \\ 
\hline
C                                                                & 199      & 161    & 0.81                           & 198      & 51     & 0.26                         & 196      & 60     & 0.31                                           \\ 
\hline
D                                                                & 198      & 138    & 0.70                           & 199      & 53     & 0.27                         & 196      & 49     & 0.25                                           \\ 
\hline
E                                                                & 195      & 146    & 0.75                           & 197      & 47     & 0.24                         & 193      & 52     & 0.27                                           \\ 
\hline
F                                                                & 198      & 173    & 0.87                           & 199      & 64     & 0.32                         & 193      & 93     & 0.48                                           \\
\hline

\end{tabular}
}
\arrayrulecolor{black}
\end{table*}


\textit{\textbf{Response \#3.1:}}
Thanks for the comment. The main objective of \FT is to generate 
a substantial number of erroneous inputs. We also highlight that the 
generated inputs are real errors (even if we do not know the ground truth 
labels). This is because, differential testing can confirm the presence 
of an error for a test when the test outputs for the two models under 
test significantly differ. Nonetheless, it is not possible to highlight 
the models that suffer from the error solely based on differential testing. 
To indicate that differential testing is a practical choice for testing 
machine-learning applications, we have added the following text in the 
revised version of the paper (\autoref{sec:overview},  paragraph on 
``Differential testing"): 
\newrevise{It is worthwhile to note that
differential testing has also been successfully used for testing ML
models in other domains~\cite{DBLP:conf/sosp/PeiCYJ17} (e.g. computer vision).}

%Finally, differential testing has also been successfully used for testing 
%ML models in other domains~\cite{deepxplore} (e.g. computer vision).}

We note that the erroneous inputs need to be labelled for retraining. 
However, it might be possible to retrain the system without the ground 
truth labels. 
We have added the following text in the revised version to clarify this 
(\autoref{sec:results}, ``Results", under $\mu$RQ, third paragraph): 
\newrevise{
It is important to note that there may be other ways 
(e.g. Transduction~\cite{learning-transduction})  to find the ground truth labels, 
but investigating such methodologies is beyond the scope 
of this work.}
We have also mentioned the following in the conclusion (\autoref{sec:conclusion})
to clarify further: \newrevise{It would also be desirable to integrate \FT with a 
system that can determine the ground truth label of the discovered inputs 
(e.g. Transduction~\cite{learning-transduction}) to effectively retrain the 
classifiers and alleviate the errors we have discovered.}

\textit{\textbf {Comment \#3.2:}
For the application to more practical benchmarks, like Google, Amazon, 
Microsoft, Baidu and etc, the authors deem they are not suitable for OGMA 
because the output does not follow a standard taxonomy. I am not fully 
convinced about this. For basic binary classification tasks, the output 
should be no problem for OGMA. Please refer to the sentiment analysis and 
toxic content detection tasks of these service providers as studied by 
TEXTBUGGER. Such experiments are crucial to demonstrate the usability of 
OGMA in practical applications. 
}

\textit{\textbf{Response \#3.2:}} Thanks for the comment. In the 
revised version of the paper, we have added a new research question: 
\newrevise{RQ6: Does \FT find errors for  different use cases and classifiers?} 
To answer this research question, we have performed additional experiments 
in the revised version of the paper and we have added our findings in 
the revised version. Concretely, we have added the following text in 
\autoref{sec:results}, ``Results" (column 1, RQ6) to discuss the new 
experimental results.

\newrevise{
To evaluate RQ6, we have evaluated the sentiment analysis tool 
provided by Google's Natural Language API \cite{google-cloud-nlp-url}. We have 
employed differential testing with Rosette's sentiment analysis service 
\cite{rosette-url}. The outputs of the Rosette API are [``POSITIVE", ``NEGATIVE", 
``NEUTRAL"]. The Google API returns a score, $sc \in (-1, 1)$ and magnitude, 
$mg \in (0, \infty)$. Using the Interpreting sentiment analysis values as a 
guide~\cite{google-nlp-interpreting-sentiments}, we classify 
the output as [``NEGATIVE"], [``NEUTRAL"] and [``POSITIVE"] when 
$sc \in (-1, -0.25]$, $~sc \in (-0.25, 0.25)$ and $sc \in [0.25, 1)$, respectively.
An input is considered an error if the outputs of the Google sentiment analysis 
API and Rosette sentiment analysis API are different. 
}


\newrevise{
We use this experiment to check OGMA’s differential testing capability. We present 
the result in Table~\ref{table:rq6-errors}. We run OGMA for 200 iterations and we evaluate 
three error discovery strategies as seen before, i.e., OGMA, random and OGMA with 
backtracking disabled. From Table~\ref{table:rq6-errors}, we observe that the results are 
in line with our findings in IAB classification use cases. Specifically, OGMA discovers 
the most number of errors, averaging an error ratio of 0.81 across the six grammars. 
The random and OGMA- No Backtrack strategies have an error ratio average of 0.29 and 
0.37, respectively.
}




\textit{\textbf {Comment \#3.3:}
After the clarification of all the technical misunderstandings, I find OGMA 
relies too much on the grammar definition. This could greatly hinder its 
application, especially on the NLP applications, because natural languages 
do not strictly follow an explicit grammar like programming languages. Even 
to list the production rules for the terminals could be a tedious task. If 
an automated algorithm is utilized to learn such a grammar, I think OGMA 
may lose the advantage of not relying on training dataset.}

\textit{
I understand that these issues regarding robustness and usability could be 
difficult to fully address. At least, I would recommend the authors discuss 
and mention the potential limitations of the proposed approach. 
}

\textit{\textbf{Response \#3.3:}} 
\FT abstracts the input space via a grammar and explores the input 
space with the objective of generating erroneous inputs. 
To clarify this aspect, we have added the following text in the 
revised version (\autoref{sec:threatsToValidity}, paragraph on 
``Complex Inputs"): \newrevise{Currently, OGMA 
only works on input domain encoded by context free grammars. This includes 
natural language processing tools (as evaluated in our work) and malware 
detectors targeting certain programming and 
scripting languages, among others. The grammar helps 
us to encode a large number of inputs and explore the input space beyond the 
training set in a systematic fashion. In our evaluation, we can easily 
construct several grammars according to a template and they facilitate in 
discovering numerous errors in the NLP classifiers.}

Nevertheless, we acknowledge our reliance on grammars for the 
effectiveness of OGMA. Thus, the threats to validity section 
(\autoref{sec:threatsToValidity}, paragraph on ``Complex Inputs") also 
includes the following text as a limitation: \newrevise{
OGMA is not evaluated on more complex input structures such as images 
and videos. To adapt our OGMA approach for such complex inputs, a model 
that encodes these inputs is needed. This can be accomplished in a 
future extension of OGMA.}



%\pagebreak
%\revise{
%To illustrate the efficacy of our retraining method, we have 
%conducted additional experiments to validate our methods. We 
%add varying percentages of discovered error data to the training 
%set. We add the discovered error data to the training data. The data
%added is measured as the percentage of the original data set. 
%As seen in \autoref{table:retrain-errors} and \autoref{fig:retrain-errors}
%the errors show a reducing trend up to 15\% and then increase. This is in
%line with the retraining trends found in other papers such as 
%\cite{aequitas}.
%}
%
%


%\revise{ https://cloud.google.com/natural-language/docs/categories
%Amazon only offers custom classification https://aws.amazon.com/comprehend/features/
%Facebook fastText does not offer classification https://github.com/facebookresearch/fastText
%Baidu only open-sourced sentiment classification system, all documentation 
%is in Chinese https://github.com/baidu/Senta
%}





